The entropy efficiency of point-push mapping classes on the punctured disk

We study the maximal entropy per unit generator of push-point mapping classes on the punctured disk. Our work is motivated by fluid mixing by rods in a planar domain. If a single rod moves among N-fixed obstacles, the resulting fluid diffeomorphism is in the push-point mapping class associated with the loop in \pi_1(D^2 - {N points}) traversed by the single stirrer. The collection of motions in each of which the stirrer goes around a single obstacle generate the group of push-point mapping classes, and the entropy efficiency with respect to these generators gives a topological measure of the mixing per unit energy expenditure of the mapping class. We give lower and upper bounds for Eff(N), the maximal efficiency in the presence of N obstacles, and prove that Eff(N) -> log(3) as N -> \infty. For the lower bound we compute the entropy efficiency of a specific push-point protocol, HSP_N, which we conjecture achieves the maximum. The entropy computation uses the action on chains in a \Z-covering space of the punctured disk which is designed for push-point protocols. For the upper bound we estimate the exponential growth rate of the action of the push-point mapping classes on the fundamental group of the punctured disk using a collection of incidence matrices and then computing the generalized spectral radius of the collection.

==> hspdefs.tex <==
%\input amssym 
%\font\deffont=cmssi10
%new for abelian

\def\Leb{Lebesgue}
\def\cF{{\cal F}}
\def\cM{{\cal M}}
\def\cFs{{\cal F}^s}
\def\cFu{{\cal F}^u}
\def\cP{{\cal P}}
\def\cI{{\cal I}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cU{{\cal U}}
\def\proof{\noindent\textbf{ Proof:}}
\def\QED{\ $\blacksquare$\smallskip}
\def\T{{\mathbb T}}
\def\bbone{\mathbbmss{1}}
\def\de#1{\textit{#1}}
\def\C{{\mathbb C}}
\def\Q{{\mathbb Q}}
\def\R{{\mathbb R}}
\def\Z{{\mathbb Z}}
\def\N{{\mathbb N}}
\def\raw{\rightarrow}
\def\per{\text{per}}
\def\uv{{\underline v}}
\def\ua{{\underline a}}
\def\uu{{\underline u}}
\def\us{{\underline s}}
\def\ut{{\underline t}}
\def\ux{{\underline x}}
\def\cS{{\cal S}}
\def\I{^{-1}}
\def\bv{{\mathbf v}}
\def\bx{{\mathbf x}}
\def\by{{\mathbf y}}
\def\Funct{\text{Func}}
\def\vn{{\vec{n}}}
\def\vm{\vec{m}}
\def\vv{\vec{v}}
\def\valpha{\vec{\alpha}}
\def\vu{\vec{u}}
\def\va{\vec{a}}
\def\vg{\vec{g}}
\def\vb{\vec{b}}
\def\vd{\vec{d}}
\def\vk{\vec{k}}
\def\vp{\vec{p}}
\def\vr{\vec{r}}
\def\vell{\vec{\ell}}
\def\tf{\tilde{f}}
\def\tY{\tilde{Y}}
\def\tg{\tilde{g}}
\def\tM{\tilde{M}}
\def\tQ{\tilde{Q}}
\def\tP{\tilde{P}}
\def\tN{\tilde{N}}
\def\tZ{\tilde{Z}}
\def\tphi{\tilde{\phi}}
\def\tpsi{\tilde{\psi}}
\def\th{\tilde{h}}
\def\htop{h_{top}}
\def\homeo{homeomorphism}
\def\homeos{homeomorphisms}
\def\diffeo{diffeomorphism}
\def\diffeos{diffeomorphisms}
\def\st{|}

\def\isomorphic{\cong}
\def\isotopic{\cong}
\def\cP{\cal{P}}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\ind}{index}
\DeclareMathOperator{\mult}{mult}
\DeclareMathOperator{\Homeo}{Homeo}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\Deck}{Deck}


\def\F{{\mathbb F}}

\def\tcF{\tilde{\cal F}}
\def\tF{\tilde{\cal F}}
\def\pA{pseudo-Anosov}


\def\tX{\tilde{X}}



\DeclareMathOperator{\rank}{rank}
\newcommand{\tensor}{\otimes}

\def\bv{{\mathbf v}}
\def\tphi{{\tilde{\phi}}}
\def\tcF{\tilde{\cal F}}
\def\tchi{{\tilde{\chi}}}
\def\tell{{\tilde{\ell}}}
\def\tH{{\tilde{H}}}
\def\tx{{\tilde{x}}}
\def\tp{{\tilde{p}}}
\def\ty{\tilde{y}}
\def\tz{{\tilde{z}}}
\def\tw{\tilde{w}}
\def\osum{\oplus}
\def\selff#1#2{#1:#2\raw #2}

\def\ie{i.e.}
\def\cf{\textit{cf.}}
\def\homega{{\hat{\omega}}}
\def\hJ{{\hat{J}}}
\def\cP{{\cal P}}
\def\cA{{\cal A}}
\def\cE{{\cal E}}
\def\cC{{\cal C}}
\def\cL{{\cal L }}
\def\tL{\tilde{L}}
%\def\allowsum{\sum_{1\leq k \leq d\atop j\raw k }}
\def\allowsum{\sum_{j\raw k }}
\def\hA{\hat{A}}
\def\hT{\hat{T}}
\def\hR{\hat{R}}
\def\htau{\hat{\tau}}
\def\hht{\hat{t}}
\def\hd{\hat{d}}
\def\hg{\hat{g}}
\def\barg{\overline{g}}
\def\hatg{\hat{g}}
\def\hS{\hat{S}}
\def\hL{\hat{L}}
\def\tR{\tilde{R}}
\def\tGamma{\tilde{\Gamma}}
\def\talpha{\tilde{\alpha}}
\def\tbeta{\tilde{\beta}}
\def\tsigma{\tilde{\sigma}}
\def\tgamma{\tilde{\gamma}}
\def\tomega{\tilde{\omega}}
\def\tiota{\tilde{\iota}}
\def\halpha{\hat{\alpha}}
\def\hbeta{\hat{\beta}}
\def\hus{\hat{\us}}
\def\hSigma{\hat{\Sigma}}
\def\hsigma{\hat{\sigma}}
\def\todo#1{$\langle\langle$\textbf{TODO: #1}$\rangle\rangle$}
\def\td{\tilde{d}}

\def\hhh{\hat{h}}
\def\normal{\vartriangleleft}
\def\hM{\hat{M}}
\def\hx{\hat{x}}
\def\hy{\hat{y}}
\def\hz{\hat{z}}
\def\vK{\mathbf{K}}
\def\PF{Perron-Fr\"obenius}
\def\hK{\hat{K}}

\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\Fix}{Fix}
\DeclareMathOperator{\fix}{Fix}
\DeclareMathOperator{\diam}{diam}


\newcommand{\fighere}[3]
{\begin{figure}[htbp]\begin{center}\includegraphics[width=#1\textwidth]{#2}
\end{center}\caption{#3}\end{figure}}

%HSP commands

\def\hgamma{\hat{\gamma}}
\def\heta{\hat{\eta}}
\DeclareMathOperator{\MCG}{MCG}
\DeclareMathOperator{\eff}{eff}
\DeclareMathOperator{\Eff}{Eff}
\DeclareMathOperator{\HSP}{HSP}
\DeclareMathOperator{\Mat}{Mat}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\SL}{SL}
\def\Hk{H^{(k)}}
\def\HN{H^{(N)}}
\def\Hko{H^{(k+1)}}
\def\Ck{C^{(k)}}
\def\posp{point-push protocol}
%\def\posp{$\pi_1$-stirring protocol}
\def\tD{\tilde{D}}
\def\tW{\tilde{Z}}
\def\tWN{\tilde{Z}_N}
\def\tWp{\tilde{Z}'}
\def\tWt{\tilde{Z}^{(2)}}
\def\tWNp{\tilde{Z}^\prime_N}
\def\tWt{\tilde{Z}^{(2)}}
\def\tWpt{\tilde{Z}^{\prime (2)}}
\def\pt{p^{(2)}}
\def\iotat{\iota^{(2)}}
\def\rhot{\rho^{(2)}}
\def\rhopt{\rho^{\prime (2)}}
\def\phit{\phi^{(2)}}
\def\ophi{\vec{\phi}}
\def\oM{\vec{M}}
\def\Tt{T^{(2)}}
\def\tht{\tilde{h}^{(2)}}
\def\thpt{\tilde{h}^{\prime (2)}}
\def\talphat{\tilde{\alpha}^{(2)}}
\def\talphapt{\tilde{\alpha}^{\prime (2)}}
\def\orho{\overline{\rho}}
\def\bn{{\mathbf n}}

\def\hHN{\hat{H}^{(N)}}
\def\hH{\hat{H}}
%\def\brhop{{\overline{\rho}^{(p)}}}
\def\brho{{\overline{\rho}}}
\def\Ak{{A^{(k)}}}
\def\bAk{{\overline{A}^{(k)}}}
\def\gsr{generalized spectral radius}
\def\jsr{joint spectral radius}
\def\uonek{{\underline{1}^{(k)}}}
\def\uonekludge{{\underline{1}^{(i-1)}}}
\def\uonekk{{\underline{1}^{(i)}}}
\def\junkk{B^{(k)}}
\def\order{\mathcal{O}}
\def\Ell{{\mathcal{L}}}
\def\wkappa{\overline{\kappa}}
\def\wGamma{\overline{\Gamma}}
\def\hGamma{\hat{\Gamma}}
\def\cbN{\overline{\mathcal{N}}}
\def\cN{{\mathcal{N}}}
\def\bN{\overline{N}}
\def\pmo{^{\pm 1}}
\def\spine{\Lambda}
\def\tspine{\tilde{\Lambda}}
\def\hDelta{{h^\Delta}}
\def\thDelta{{\tilde{h}^\Delta}}
\def\tspinet{\tilde{\Lambda}^{(2)}}
\def\tspinept{\tilde{\Lambda}^{\prime (2)}}
\def\tchit{\tilde{\chi}^{(2)}}
\def\tchipt{\tilde{\chi}^{\prime (2)}}
\def\tphit{\tilde{\phi}^{(2)}}
\def\tchi{\tilde{\chi}}
\def\fmh{fluid motion diffeomorphism}
\def\uell{{\underline{\ell}}}

